Online Submodular Welfare Maximization: Greedy Beats 1/2 in Random Order

In the Submodular Welfare Maximization (SWM) problem, the input consists of a set of $n$ items, each of which must be allocated to one of $m$ agents. Each agent $\ell$ has a valuation function $v_\ell$, where $v_\ell(S)$ denotes the welfare obtained by this agent if she receives the set of items $S$. The functions $v_\ell$ are all submodular; as is standard, we assume that they are monotone and $v_\ell(\emptyset) = 0$. The goal is to partition the items into $m$ disjoint subsets $S_1, S_2, \ldots S_m$ in order to maximize the social welfare, defined as $\sum_{\ell = 1}^m v_\ell(S_\ell)$. In this paper, we consider the online version of SWM. Here, items arrive one at a time in an online manner; when an item arrives, the algorithm must make an irrevocable decision about which agent to assign it to before seeing any subsequent items. This problem is motivated by applications to Internet advertising, where user ad impressions must be allocated to advertisers whose value is a submodular function of the set of users / impressions they receive. In the random order model, the adversary can construct a worst-case set of items and valuations, but does not control the order in which the items arrive; instead, they are assumed to arrive in a random order. Obtaining a competitive ratio of $1/2 + \Omega(1)$ for the random order model has been an important open problem for several years. We solve this open problem by demonstrating that the greedy algorithm has a competitive ratio of at least $0.505$ for the Online Submodular Welfare Maximization problem in the random order model. For special cases of submodular functions including weighted matching, weighted coverage functions and a broader class of "second-order supermodular" functions, we provide a different analysis that gives a competitive ratio of $0.51$.

==> Conjecture-short.tex <==
%\documentclass{article}
%
%\usepackage{amsthm}
%
%\newtheorem{theorem}{Theorem} %\newtheorem{lemma}{Lemma}
%\newtheorem{conjecture}{Conjecture}



%\begin{document}

While the techniques of the previous section show that the competitive
ratio of the Greedy algorithm is strictly better than $1/2$, we
believe that the performance is considerably better. In this section,
we present a natural conjecture on the marginal increases in welfare
obtained by Greedy (Conjecture~\ref{Conjecture:MarginalGains}), that
captures much of the difficulty of this problem.
Theorem~\ref{Thm:Greedy0.567}, proved in the full version of this
paper, shows that if the conjecture holds, the Greedy algorithm
achieves at least a competitive ratio of $0.567$. In order to state
the conjecture, we need to introduce some notation:

\begin{definition}
  Fix a permutation $\pi = (\pi_1, \pi_2, \cdots, \pi_n)$. We define
  two new permutations based on $\pi$:
  \begin{itemize}
  \item Let $\pi^{Move,i}$ be the permutation $(\pi_1, \pi_2, \cdots,
    \pi_{i-1}, \pi_{i+1}, $ $\pi_{i+2}, \cdots, \pi_n, \pi_i)$ (which is
    achieved from $\pi$ by moving $\pi_i$ to the end).
  \item Let $\pi^{Copy,i}$ be the permutation $(\pi_1, \pi_2, \cdots,
    \pi_{n}, \pi_i)$ (achieved from $\pi$ by copying $\pi_i$ to the
    end without removing the original $\pi_i$). We note that
    $\pi^{Copy,i}$ is a sequence of $n+1$ items with two copies of
    item $\pi_i$.
  \end{itemize}
\end{definition}

%Let $\pi$ denote the arrival order of the $n$ online items; note that
%in the random order model, $\pi$ is a random variable. 

Let $MG(i, \pi)$ denote the marginal gain that the algorithm Greedy
gets by allocating the $i$th online item $\pi_i$ in permutation $\pi$,
and let $\mathbb{S}_n$ be the set of all $n!$ permutations on the $n$
items.  The algorithm Greedy achieves welfare
$\textit{Welfare}(Greedy) = \mathbb{E}_{\pi \sim
  \mathbb{S}_n}[\sum_{i=1}^n MG(i,\pi)]$ where the expectation is
taken over permutations $\pi$ chosen uniformly at random from
$\mathbb{S}_n$.  
%
It is clear that $MG(i, \pi) \geq MG(n,\pi^{Move,i})$ for any $\pi$
since the first $i-1$ items of both $\pi$ and $\pi^{Move,i}$ are the
same, and therefore Greedy's allocation on them is the same; the claim
is implied by the non-increasing marginals property of submodular
functions.  Now we can present the conjecture, and the improved
competitive ratio for greedy based on it:

\begin{conjecture}\label{Conjecture:MarginalGains}
  For any instance of the online submodular welfare maximization
  problem, we conjecture that
  \[\mathbb{E}_{\pi \sim
    \mathbb{S}_n}\left[\sum_{i=1}^n MG(n+1, \pi^{Copy,i})\right] \le
  \mathbb{E}_{\pi \sim \mathbb{S}_n}\left[\sum_{i=1}^n MG(n,
  \pi^{Move,i})\right].\]
  We also note that the latter is equal to
  $n\mathbb{E}_{\pi \sim \mathbb{S}_n}[MG(n,\pi)]$ as both $\pi$ and
  $\pi^{Move,i}$ have the same distribution.
\end{conjecture}


\begin{theorem}\label{Thm:Greedy0.567} 
  Assuming Conjecture~\ref{Conjecture:MarginalGains} holds, the
  competitive ratio of the Greedy algorithm for \oswm is at least
  $0.567$ in the random order model.
\end{theorem}

%\end{document}

















































